What is an OS?

While the engineering of operating systems is well understood, their formal structure and properties are not. The latter needs a clear definition of the purpose of an OS and an identification of the core. In this paper I offer definitions of the OS, processes and files, and present a few useful principles. The principles allow us to identify work like closure and continuation algorithms, in programming languages that is useful for the OS problem. The definitions and principles should yield a symbolic, albeit semiquantitative, framework that encompasses practice. Towards that end I specialise the definitions to describe conventional OSes and identify the core operations for a single computer OS that can be used to express their algorithms. The assumptions underlying the algorithms offer the design space framework. The paging and segmentation algorithms for conventional OSes are extracted from the framework as a check. Among the insights the emerge is that an OS is a constructive proof of equivalence between models of computation. Clear and useful definitions and principles are the first step towards a fully quantitative structure of an OS.

==> Makefile <==
#
# Operating Systems paper
#
### Directory Structure
TOP=$(shell pwd)
SRCDIR=$(TOP)
BLDDIR=$(TOP)
OUTDIR=$(TOP)
IMGDIR=$(TOP)
FIGDIR=$(IMGDIR)
EPSDIR=$(IMGDIR)
IMGOUTDIR=$(IMGDIR)

### Commands and options (if any)
#LATEX=pdflatex
TODAY=$(shell date +%d-%m-%Y-%H-%M-%S)
DVIPS=dvips
LATEX=latex
DVIPDF=dvipdf
PS2PDF=ps2pdf
BIBTEX=bibtex
LATEXOPTS=-interaction=batchmode -output-directory=$(BLDDIR)

# For WIOS style
WIOSNAME=wios
WIOSBIBFILE=$(SRCDIR)/refs.bib
WIOSBIBDATA=$(SRCDIR)/$(WIOSNAME).bbl
WIOSSOURCES=$(SRCDIR)/$(WIOSNAME).tex
WIOSMAINTEX=$(BLDDIR)/$(WIOSNAME).tex

WIOSDVIOUT=$(WIOSNAME).dvi
WIOSPSOUT=$(WIOSNAME).ps
WIOSPDFOUT=$(WIOSNAME).pdf

WIOSAUX=$(WIOSNAME).aux
WIOSTOC=$(WIOSNAME).toc
WIOSLOG=$(WIOSNAME).log
WIOSFIG=$(WIOSNAME).lof
WIOSTAB=$(WIOSNAME).lot
WIOSBRF=$(WIOSNAME).brf

# Targets
default: all

all: wios

# WIOS Target
wios: $(WIOSPDFOUT)
	@echo "Done."

$(WIOSPDFOUT): $(WIOSPSOUT)
	@echo -n "-> Generating PDF from `basename $(WIOSPSOUT)`  ... "   && \
	cd $(BLDDIR)                                                      && \
	$(PS2PDF) $(WIOSPSOUT) $(WIOSPDFOUT)                              && \
	cd $(TOP)                                                         && \
	echo "Done."

$(WIOSPSOUT): $(WIOSDVIOUT)
	@echo -n "-> Generating PS  from `basename $(WIOSDVIOUT)` ... "   && \
	cd $(BLDDIR)                                                      && \
	$(DVIPS) -q $(WIOSDVIOUT) -o $(WIOSPSOUT)                         && \
	cd $(TOP)                                                         && \
	echo "Done."

$(WIOSDVIOUT): prepare passone passtwo passthree
	@echo "-> DVI Done."

prepare:
	@echo "-> Generating DVI from `basename $(WIOSMAINTEX)` ... "

passone: $(WIOSSOURCES)
	@echo -n "->   Pass 1 ... "                                       && \
	cd $(BLDDIR)                                                      && \
	$(LATEX)  $(LATEXOPTS) $(WIOSMAINTEX) > /dev/null                 && \
	echo "Done."                                                      || \
	(less $(BLDDIR)/$(WIOSNAME).log                                   && \
	echo -e "\n** Log file: $(BLDDIR)/$(WIOSNAME).log"                && \
	/bin/false)
	@cd $(TOP)

passtwo: $(BLDDIR)/$(WIOSDVIOUT)
	@echo -n "->   Pass 2 ... "                                       && \
	cd $(BLDDIR)                                                      && \
	$(LATEX)  $(LATEXOPTS) $(WIOSMAINTEX) > /dev/null                 && \
	echo "Done."                                                      || \
	(less $(BLDDIR)/$(WIOSNAME).log                                   && \
	echo -e "\n** Log file: $(BLDDIR)/$(WIOSNAME).log"                && \
	/bin/false)
	@cd $(TOP)

passthree: $(BLDDIR)/$(WIOSDVIOUT)
	@echo -n "->   Pass 3 ... "                                       && \
	cd $(BLDDIR)                                                      && \
	$(LATEX)  $(LATEXOPTS) $(WIOSMAINTEX) > /dev/null                 && \
	echo "Done."                                                      || \
	(less $(BLDDIR)/$(WIOSNAME).log                                   && \
	echo -e "\n** Log file: $(BLDDIR)/$(WIOSNAME).log"                && \
	/bin/false)
	@cd $(TOP)

# Maintenance targets

clean:
	/bin/rm -f                   \
	   $(BLDDIR)/$(WIOSDVIOUT)   \
	   $(BLDDIR)/$(WIOSAUX)      \
	   $(BLDDIR)/$(WIOSLOG)      \
	   $(BLDDIR)/$(WIOSTOC)      \
	   $(BLDDIR)/$(WIOSFIG)      \
	   $(BLDDIR)/$(WIOSTAB)      \
	   $(BLDDIR)/$(WIOSBRF)      \
	   $(BLDDIR)/$(WIOSPSOUT)    \
	   $(BLDDIR)/$(WIOSPDFOUT)   \
	   $(BLDDIR)/*~

help:
	@echo
	@echo "Usage: make {clean|texclean|help}"
	@echo "   No arguments:    Build the PDF version of the paper"
	@echo "   clean:           Remove everything that we generate"
	@echo "   texclean:        Remove everything that TeX generates"
	@echo "   help:            This help"
	@echo

